BLiRF: Bandlimited Radiance Fields for Dynamic Scene Modeling

Reasoning the 3D structure of a non-rigid dynamic scene from a single moving camera is an under-constrained problem. Inspired by the remarkable progress of neural radiance fields (NeRFs) in photo-realistic novel view synthesis of static scenes, extensions have been proposed for dynamic settings. These methods heavily rely on neural priors in order to regularize the problem. In this work, we take a step back and reinvestigate how current implementations may entail deleterious effects, including limited expressiveness, entanglement of light and density fields, and sub-optimal motion localization. As a remedy, we advocate for a bridge between classic non-rigid-structure-from-motion (\nrsfm) and NeRF, enabling the well-studied priors of the former to constrain the latter. To this end, we propose a framework that factorizes time and space by formulating a scene as a composition of bandlimited, high-dimensional signals. We demonstrate compelling results across complex dynamic scenes that involve changes in lighting, texture and long-range dynamics.

==> tab-quant-dnerf.tex <==
\begin{table*}[htbp]
    \centering
    % \footnotesize
    \small
    \ra{1.1}
    \renewcommand\tabcolsep{4pt}
    \begin{tabularx}{\textwidth}{lcccccccccccccccc}
        \toprule
        && \multicolumn{3}{c}{Bouncing Balls} && \multicolumn{3}{c}{Hell Warrior} && \multicolumn{3}{c}{Hook} && \multicolumn{3}{c}{Jumping Jacks} \\
        Method && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
        \cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} \cmidrule{15-17}
        TensoRF && 20.70 & 0.91 & 0.19 && 13.17 & 0.75 & 0.31 && 16.23 & 0.83 & 0.21 && 18.44 & 0.87 & 0.22  \\
        T-TensoRF && - & - & - && - & - & - && - & - & - && - & - & -  \\
        D-NeRF && 38.93 & 0.99 & 0.10 && 25.03 & 0.95 & 0.07 && 29.26 & 0.96 & 0.12 && 32.81 & 0.98 & 0.04  \\
        NR-NeRF && 24.65 & 0.96 & 0.14 && 12.59 & 0.84 & 0.27 && 19.40 & 0.92 & 0.18 && 24.17 & 0.95 & 0.18  \\
        Ours && - & - & - && - & - & - && - & - & - && - & - & -  \\

        \midrule
        % \\
        && \multicolumn{3}{c}{Lego} && \multicolumn{3}{c}{Mutant} && \multicolumn{3}{c}{Stand Up} && \multicolumn{3}{c}{T-Rex} \\
        Method && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
        \cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} \cmidrule{15-17}
        TensoRF && 20.32 & 0.89 & 0.13 && 19.76 & 0.91 & 0.10 && 17.71 & 0.88 & 0.16 && 23.91 & 0.93 & 0.09  \\
        T-TensoRF && - & - & - && - & - & - && - & - & - && - & - & -  \\
        D-NeRF && 21.64 & 0.84 & 0.17 && 31.29 & 0.97 & 0.03 && 32.80 & 0.98 & 0.02 && 31.76 & 0.98 & 0.04  \\
        NR-NeRF && - & - & - && 25.15 & 0.96 & 0.14 && 21.61 & 0.95 & 0.17 && 24.17 & 0.94 & 0.16  \\
        Ours && - & - & - && - & - & - && - & - & - && - & - & -  \\

        \bottomrule
    \end{tabularx}
    % \end{tabular}
    \caption{Quantitative comparison of novel view synthesis on D-NeRF dataset\cite{pumarola2021d}. We report the average PSNR, SSIM (higher is better) and LPIPS (lower is better) results. Best results are in bold.}
    \label{tab:quant-dnerf}
\end{table*}
